Fast, Cheap, and Fair? Evaluating Decision Models

Industries are increasingly adopting AI-driven systems to automate a wide range of tasks, including high-stakes decisions in human resources, such as candidate screening and recruitment. This makes evaluating their fairness essential, particularly when decisions directly affect individuals' opportunities. Accordingly, the EU AI Act classifies recruitment AI systems as high-risk, imposing strict requirements on their deployment. In this context, compact ``System~1'' decision models offer a fast and cost-efficient alternative to general-purpose LLMs, yet their fairness remains largely unexplored. This article presents the first systematic bias and fairness audit of \jev{}, a typed-decision model targeting recruitment applications. The study evaluates how explicit demographic attributes and implicit candidate cues influence screening scores, rankings, and shortlisting outcomes. These effects are compared against a noise floor derived from name substitutions and typographical variations. The evaluation also examines output validity, latency, and cost. Counterfactual CV datasets and evaluation code are released for reproducibility.

==> macros.tex <==
% ============================================================================
% macros.tex -- single source of truth for names and notation.
% \input{macros} in the preamble, after \usepackage{amsmath,amssymb,booktabs}.
% Safe to load after other definitions: every macro is defined with
% \providecommand{}\renewcommand, so it overrides any earlier definition
% instead of raising "Command already defined". Load it LAST in the preamble.
% Rule: never type a model, dataset, attribute or metric name directly in the
% text or tables; always use the macro, so a rename is a one-line change.
% ============================================================================
\RequirePackage{xspace}
\usepackage[inline]{enumitem}

% ---------------------------------------------------------------- model names
% Product names in plain roman (\textnormal keeps them upright in math too). Versions appear once, in Table~\ref{tab:models}.
\providecommand{\jev}{}\renewcommand{\jev}{\textnormal{JEV}\xspace}
\providecommand{\laya}{}\renewcommand{\laya}{\textnormal{Laya}\xspace}
\providecommand{\luna}{}\renewcommand{\luna}{\textnormal{GPT-6 Luna}\xspace}
\providecommand{\sol}{}\renewcommand{\sol}{\textnormal{GPT-6.1 Sol}\xspace}
% Model families: defined terms, always capitalised.
\providecommand{\dm}{}\renewcommand{\dm}{Decision Model\xspace}
\providecommand{\dms}{}\renewcommand{\dms}{Decision Models\xspace}
\providecommand{\gm}{}\renewcommand{\gm}{Generative Model\xspace}
\providecommand{\gms}{}\renewcommand{\gms}{Generative Models\xspace}
% \newcommand{\gms}{Generative Models\xspace}

% Short forms, for tables only.
\providecommand{\dmshort}{}\renewcommand{\dmshort}{Dec.\xspace}
\providecommand{\gmshort}{}\renewcommand{\gmshort}{Gen.\xspace}

% ---------------------------------------------------------------- dataset names
\providecommand{\dscf}{}\renewcommand{\dscf}{\textsc{hiring-fairness}\xspace}         % counterfactual CV screening (Kaggle part of Seshadri et al.)
\providecommand{\dsfit}{}\renewcommand{\dsfit}{\textsc{JD-Fit}\xspace}       % resume-job-description-fit
% \providecommand{\dsdiscrim}{}\renewcommand{\dsdiscrim}{\textsc{discrim-eval}\xspace}      % Tamkin et al. (official name, never renamed)

% ---------------------------------------------------------------- attributes, groups, signals
\providecommand{\attr}{}\renewcommand{\attr}[1]{\textsc{#1}}                 % \attr{gender}, \attr{ethnicity}, \attr{origin}
\providecommand{\gender}{}\renewcommand{\gender}{\attr{gender}\xspace}
\providecommand{\ethnicity}{}\renewcommand{\ethnicity}{\attr{ethnicity}\xspace}
\providecommand{\origin}{}\renewcommand{\origin}{\attr{origin}\xspace}
\providecommand{\gender}{}\providecommand{\demographic}{\attr{demographic}\xspace}
\providecommand{\sexp}{}\renewcommand{\sexp}{\textsc{exp}}                   % explicit signal
\providecommand{\simp}{}\renewcommand{\simp}{\textsc{imp}}                   % implicit (name) signal

% ---------------------------------------------------------------- notation
% Rules (see also Sec. 3.1):
%  (i)   scalars, indices, single elements: lowercase italic        n, k, s, g
%  (ii)  documents and sets: uppercase italic                         J, C, P_j, G_a
%  (iii) vectors: bold lowercase                                       \vect{s}, \vect{w}
%  (iv)  matrices: bold uppercase                                      \mat{S}
%  (v)   entries: numeric subscripts in square brackets               \mat{S}_{[i,g]}
%  (vi)  domains / spaces: calligraphic                               \cJ, \cC, \cA
\providecommand{\vect}{}\renewcommand{\vect}[1]{\mathbf{#1}}
\providecommand{\mat}{}\renewcommand{\mat}[1]{\mathbf{#1}}
\providecommand{\cJ}{}\renewcommand{\cJ}{\mathcal{J}}                      % domain of job descriptions
\providecommand{\cC}{}\renewcommand{\cC}{\mathcal{C}}                      % domain of CVs
\providecommand{\cA}{}\renewcommand{\cA}{\mathcal{A}}                      % set of bias attributes
\providecommand{\cM}{}\renewcommand{\cM}{\mathcal{M}}                      % set of models
\providecommand{\cS}{}\renewcommand{\cS}{\mathcal{S}}                      % discrim-eval scenarios
\providecommand{\cf}{}\renewcommand{\cf}[3]{C^{(#1,#2,#3)}}                % counterfactual version: \cf{a}{g}{\sigma}
\providecommand{\gref}{}\renewcommand{\gref}[1]{g^{0}_{#1}}                  % reference group of attribute #1
\providecommand{\ins}{}\renewcommand{\ins}{\oplus}                          % line-insertion operator

% ---------------------------------------------------------------- metrics (same names as in the tables)
\providecommand{\dscore}{}\renewcommand{\dscore}{\Delta\mathrm{Score}}
\providecommand{\drank}{}\renewcommand{\drank}{\Delta\mathrm{Rank}}
\providecommand{\excl}{}\renewcommand{\excl}{\mathrm{Excl@5}}
\providecommand{\disag}{}\renewcommand{\disag}{\mathrm{Disag@5}}
\providecommand{\dauc}{}\renewcommand{\dauc}{\Delta\mathrm{AUC}}
\providecommand{\pyes}{}\renewcommand{\pyes}{p(\mathrm{yes})}
\providecommand{\logit}{}\renewcommand{\logit}{\mathrm{logit}}
\providecommand{\sig}{}\renewcommand{\sig}{$^{*}$}                          % significance marker in tables



\newcommand{\ci}[2]{{\scriptsize[#1,\,#2]}}

